Bright 4B: Scaling Hyperspherical Learning for Segmentation in 3D Brightfield Microscopy

Label-free 3D brightfield microscopy offers a fast and noninvasive way to visualize cellular morphology, yet robust volumetric segmentation still typically depends on fluorescence or heavy post-processing. We address this gap by introducing Bright-4B, a 4 billion parameter foundation model that learns on the unit hypersphere to segment subcellular structures directly from 3D brightfield volumes. Bright-4B combines a hardware-aligned Native Sparse Attention mechanism (capturing local, coarse, and selected global context), depth-width residual HyperConnections that stabilize representation flow, and a soft Mixture-of-Experts for adaptive capacity. A plug-and-play anisotropic patch embed further respects confocal point-spread and axial thinning, enabling geometry-faithful 3D tokenization. The resulting model produces morphology-accurate segmentations of nuclei, mitochondria, and other organelles from brightfield stacks alone--without fluorescence, auxiliary channels, or handcrafted post-processing. Across multiple confocal datasets, Bright-4B preserves fine structural detail across depth and cell types, outperforming contemporary CNN and Transformer baselines. All code, pretrained weights, and models for downstream finetuning will be released to advance large-scale, label-free 3D cell mapping.

==> sec/1_intro_OG.tex <==
\section{Introduction}
\label{sec:intro}


% \begin{figure}[t] % The asterisk* makes it span columns, [t] places it at the top
%   \centering % Center the figure horizontally
%   \includegraphics[width=1\linewidth]{sec/figs/PAGE1.pdf} % Or .png, .jpg
%   \caption{\textit{Brightfield to Structure Segmentation.} Bright 4B is a 3D-native, feed-forward transformer that ingests a single brightfield stack and outputs morphology-accurate structure segmentations in one pass, without post-processing or test-time optimization. The above 3D visualizations are the raw network output without any postprocessing except a fixed threshold of 80 percent.}
%   \label{fig:coverphoto} % Label for referencing the figure in text
% \end{figure}

% \bsm{A 4-B-parameter model trained on microscopy data raises practical questions for the CVPR reviewers -- such as 

% How much data is available? 10TB

% Was training from scratch or using self-supervised pretraining?
% from scratch

% How long did it take, on what hardware?

% CVPR reviewers will expect reproducibility and realistic compute claims. so you should address the scalability/feasibility upfront. Dont recall seeing a discussion on this.}

% \begin{figure}
%     \centering
%     \includegraphics[width=1\linewidth]{sec/figs/image (11).png}
%     \caption{\textit{Brightfield to Nuclei Segmemtation}}
%     \label{fig:placeholder}
% \end{figure}


\begin{figure}
    \centering
    \includegraphics[width=0.7
    \linewidth]{sec/figs/PATCH.jpg}
    \caption{\textbf{Anisotropic 3D patch embedding.} We first apply a PSF-aware depthwise axial low-pass with stride $p_z$ to prevent aliasing, yielding $(B, C, D/p_z, H, W)$. We then tile the $XY$ plane into $p_y \times p_x = 16\times16$ blocks and fold each tile (across channels) into a vector of length ($p_y p_x$). A bias-free projection maps each vector to (h) dimensions, producing a geometry-faithful token lattice ($(B, D', H', W', h)$) with ($D' = D/2$). Crucially, $p_z$ does not inflate the token dimension; axial decimation is handled by the anti-alias conv, while token content remains $(16\times16)$. This $(2\times16\times16)$ design respects confocal anisotropy and reduces block artifacts, yielding accurate boundaries in downstream 3D segmentation.}
    \label{fig:placeholder}
\end{figure}
% \bsm{intro is good but not quite in the CVPR framework. it is also a bit dense. have reworded and broken the paragraphs for better readability. commenting out the older paras so you can go back as needed.}

%We are currently at the point in time where billion parameter models are prevalent \textit{and} successful at solving 2D vision problems, and yet we simply are not pushing the boundaries of these large models into solving 3D and beyond problems. A current bottleneck is the lack of architectures other than ViT with high quality pretrained weights---specifically architectures that are inherently 3D, not pseudo-3D, \ie processing slice by slice. 

We are at a point where billion-parameter models have become both prevalent and remarkably effective in solving 2D vision tasks, yet their potential for 3D understanding remains largely untapped. A key bottleneck lies in the scarcity of architectures---beyond ViT---that provide high-quality pretrained weights and are \emph{natively 3D}, rather than pseudo-3D models that process slices independently.

Building on the success of Vision Transformers and recent advances in the natural language processing (NLP) community, we revisit the transformer design through the lens of volumetric data flow \cite{elhage2021mathematical}. We begin with an \emph{anisotropic 3D patch embed} that low-passes and strides only along $z$ (point-spread function (PSF)–aware) while maintaining native in-plane resolution. This produces a depth-indexed lattice of planar tokens $(D'\!\times\!H\!\times\!W)$ that preserves fine $xy$ detail and mitigates aliasing along the thin axial dimension. Within each block, we replace dense self-attention with \emph{Native Sparse Attention (NSA)} \cite{yuan2025native}, which routes information through three complementary paths: (i) a local in-plane sliding window that preserves boundaries and suppresses clutter, (ii) a coarse compressive pathway (a compact Transformer over depth summaries) that supplies denoised long-range context, and (iii) a selected global pathway that attends to a sparse set of salient regions across the volume. Conceptually, NSA performs an information triage across three orthogonal subspaces---local planar structure, coarse cross-slice regularities, and sparse global correspondences---so model capacity scales adaptively with the structure of the data. A learned per-head mixer weights these paths, while grouped queries reduce key-value redundancy for efficiency.

\sm{We leverage this new architecture to improve the label-free prediction of organelles from 3D bright field images acquired with 3D spinning disk confocal}. Since our primary objective is to learn 3D subcellular representations, we make stable representation learning the core design principle. Unit-normalizing all token states and projections constrains updates to the unit hypersphere, yielding numerically stable behavior even at the billion-parameter scale. Attention and feed-forward blocks are wrapped with \emph{HyperConnections}, wherein multiple residual streams with learned width and depth gates softly interpolate pre- and post-update states, preserving priors while allowing deeper layers to inject new information. Finally, the feed-forward is replaced with a \emph{soft Mixture-of-Experts (MoE)} employing load-balanced, slot-based routing, enabling experts to specialize (\eg, boundary sharpening, texture suppression, global morphology). Intermediate features are exposed to a UNETR-style decoder for volumetric segmentation.

%Inspired by the success of Vision Transformer and recent advances in the natural language processing (NLP) field, we took apart the original design and scrutinized how information flow would work as 3D data was processed throughout the subspaces \cite{elhage2021mathematical}. To do this, we begin with an \emph{anisotropic 3D patch embed} that low–passes and strides only along $z$ (point-spread function (PSF)–aware) while keeping native in–plane resolution. This yields a depth-indexed lattice of planar tokens $(D'\!\times\!H\!\times\!W)$ that preserves fine $xy$ detail and avoids aliasing along the thin axial dimension. Next, we moved inside each block and replaced dense self–attention with \emph{Native Sparse Attention (NSA)} \cite{yuan2025native}, which routes information along three complementary paths: (i) a local in–plane sliding window that preserves boundaries and suppresses background clutter, (ii) a coarse compressive pathway (a tiny Transformer over depth–summaries) that supplies long–range but denoised cross–slice context, and (iii) a selected global pathway that attends to a small set of salient regions across the volume. Conceptually, NSA implements an information triage that mirrors three orthogonal subspaces---local planar structure, coarse cross–slice regularities, and sparse global correspondences---so capacity scales where the data demands it. A learned mixer per head weights these paths, while grouped queries reduce key-value (KV) redundancy. And, since the main goal of this paper is to effectively learn how to segment subcellular structures in 3D, we make representation learning our guiding light for architectural decisions. We find that unit-normalizing all token states and projections so updates move on a hypersphere enables stable representation at the billion parameter scale. We wrap attention and feed-forwards with HyperConnections---wherein multiple residual streams with learned width/depth gates softly interpolate pre and post–update states, retaining useful priors while allowing depth to add information. Finally, the feed–forward is a \emph{soft mixture-of-experts (MoE)} with load–balanced, slot–based routing so experts specialize (\eg, boundary sharpening, texture suppression, global shape). Features are exposed at selected depths to a UNETR decoder.  

% This factorization implicitly answers \emph{why} a 4B–parameter model is warranted: multi–head attention and MoE allocate a large but \emph{conditional} parameter budget to diverse brightfield “circuits” (in the Transformer–circuits sense) without collapsing them into a single pathway, enabling the model to span the high–variance morphology manifold while keeping per–token compute tractable.


%\textit{Why focus only on brightfield?} Because brightfield microscopes are fast, gentle, and everywhere, but accurate 3D masks still usually require fluorescence, multi-channel acquisition, or heavy post-processing. This gap limits high-throughput studies \cite{viana2023integrated} where labeling is costly or infeasible and where phototoxicity needs to be minimized. Modern vision transformers \cite{dosovitskiy2020image,dehghani2023scaling,zhai2022scaling} scale well and can model long-range 3D context, yet off-the-shelf designs struggle with anisotropic axial sampling, brightfield-specific artifacts (halos, uneven illumination), and the need to balance local edges with global morphology under tight memory budgets. Prior work either assumes fluorescence supervision \cite{kraus2024masked} or relies on pipelines that stitch many heuristics together \cite{pachitariu2025cellpose, stringer2021cellpose,hatamizadeh2022unetr}. A single, end-to-end model that segments subcellular structures directly from brightfield volumes remains elusive. 
\paragraph{Why focus only on brightfield?} Brightfield microscopy is fast, gentle, and nearly ubiquitous, yet accurate 3D segmentation still typically requires fluorescence, multi-channel acquisition, or extensive post-processing. This limitation hinders high-throughput cell studies \cite{viana2023integrated}, where labeling is costly, phototoxicity must be minimized, and throughput is essential. Modern vision transformers \cite{dosovitskiy2020image,dehghani2023scaling,zhai2022scaling} scale effectively and capture long-range 3D context, but off-the-shelf architectures struggle with anisotropic axial sampling, brightfield-specific artifacts (halos, uneven illumination), and the trade-off between preserving local edges and modeling global morphology under tight memory constraints. Prior work has either relied on fluorescence supervision \cite{kraus2024masked} or assembled heuristic multi-stage pipelines \cite{pachitariu2025cellpose,stringer2021cellpose,hatamizadeh2022unetr}. %To date, a single end-to-end model capable of segmenting subcellular structures directly from raw brightfield volumes—without auxiliary channels or handcrafted processing—has remained out of reach. 
\sm{To date, label-free approaches have primarily focused on predicting fluorescent organelle images from bright-field. However, this method requires a secondary, downstream step of segmenting the predicted fluorescent images. This work, therefore, proposes a more direct approach: we learn to generate organelle segmentations straight from the bright-field images, bypassing the intermediate image-to-image translation.}

Hence, our goal is to build a \textit{foundation model for segmenting subcellular structures in 3D brightfield microscopy}. We define a foundation model as a high-capacity network trained on large-scale, domain-specific data---in this case, brightfield volumes---that serves as a transferable initialization for subsequent tasks. Such a model should accelerate convergence and improve generalization when adapted to downstream objectives, whether through continued pretraining or finetuning on smaller datasets for segmentation or classification.

We make the following contributions:
\begin{enumerate}
    \item \textbf{Bright-4B architecture.} We introduce \textit{Bright-4B}, a 4B-parameter 3D vision architecture for target segmentation from brightfield images that learns subcellular representations on the unit hypersphere. It integrates hardware-aligned \emph{Native Sparse Attention} for multi-scale spatial context and a normalized \emph{Soft Mixture-of-Experts} for adaptive capacity. We show that constraining all residual and expert updates to the unit hypersphere stabilizes billion-parameter training, resolving the instability traditionally associated with normalized Mixture-of-Experts.

    \item \textbf{Label-free 3D segmentation.} Given a single 3D brightfield stack, Bright-4B produces segmentations of subcellular structures (\ie nucleoli, mitochondria, nuclei, golgi) without auxiliary fluorescence channels or post-processing. We provide eight structure-specific models that can be used directly or finetuned for downstream applications. \sm{As expected, the model's accuracy is organelle-dependent. This directly reflects the amount of physical information present in the bright-field image, which is dictated by each organelle's refractive index and size. Despite this inherent physical limitation, our results show that the models are highly robust and hold significant potential for downstream analysis.}
    
    \item \textbf{Open foundation for microscopy AI.} All pretrained weights, code, and training recipes will be released to enable community reuse, benchmarking, and further scaling of label-free 3D foundation models.

\end{enumerate}

% \bsm{the novelty claim is about integration, adaptation, or domain alignment rather than invention of those modules. make this clear. } 

% \ak{But I did modify the residual connection and MoE methods to work with my learning on the hypersphere claim. This actually deviates away from the literature that states noralizing MoE hurts the performance and makes it unstable. We fixed this by keeping everything on the hypersphere, that's how we solved the instability issue in MoE and learned depth and width residual connections. Nobody in the literature has done this. How do I sell this as a novelty?}

%%We make all of our code and models publicly available at \texttt{github link.}
%%BSM moved to the item above.

%%=========
%% addressing the modifications part here.

Unlike prior Mixture-of-Experts (MoE) models, where normalization disrupts routing dynamics and destabilizes large-scale training, \textbf{Bright-4B} reformulates both attention and expert computation on the \textit{unit hypersphere}. All token states and projections are L2-normalized so that updates act as rotations rather than rescalings. This hyperspherical constraint eliminates gradient explosion and expert collapse—common in normalized MoE—enabling stable optimization at the 4B-parameter scale. To our knowledge, this is the first demonstration that hyperspherical normalization can \emph{stabilize} sparse expert models while retaining expert specialization.



% \bsm{be explicit that your novelty lies in the domain-aligned integration (PSF-aware tokenization + normalized transformer stack) rather than introducing new attention or MoE mechanics. Make this into a bulleted list. You can also be very specific about the integration of advanced modules (NSA, MoE, DHC etc.) here.}

% \bsm{Positioning and Motivation need to be clearer for the CVPR Audience. 

% 1. The introduction needs stronger connection to computer vision rather than microscopy per se.

% 2. The paper should explicitly frame brightfield microscopy as an important low-contrast, physics-limited vision domain that pushes generalizable 3D representation learning. May not be obvious for a generic CVPR researcher.

% 3.  “foundation model” must be substantiated: Is this truly foundation-scale (multi-task, cross-structure pretraining), or just a large architecture trained per task? Not clear to me what is "foundational".

% }
% \ak{Foundation model means a model that can be finetuned for multiple downstream tasks using a well trained backbone. Our model has seen thousands of brightfield images, making it robust for downstream tasks. }


==> sec/2_relatedworks_OG.tex <==
\section{Related Work}
\label{sec:relatedworks}

% \bsm{It should reference biological imaging efforts in label-free reconstruction and physics-informed learning in greater depth and relate them conceptually to foundation-model trends (MAE, SAM-style pretraining, etc.).

% Also, clarify how this differs from Cellpose-SAM (Pachitariu et al., 2025) beyond being 3D and brightfield-only.}


%\paragraph{Label-free prediction and nuclear segmentation.}
%Early work on label-free fluorescence prediction learned direct mappings from transmitted-light images to fluorescent channels using CNNs \cite{christiansen2018silico,ounkomol2018label,rivenson2019phasestain}. While effective in 2D, these approaches struggle in 3D brightfield where axial blur and signal ambiguity increase with depth. Instance segmentation methods such as Cellpose \cite{stringer2021cellpose} variants have brightfield models, but often rely on strong priors, 2D processing, or post-hoc tracking to recover 3D nuclei. Our problem setting is stricter: we predict \emph{3D subcellular structure masks from brightfield alone}, end-to-end, with no auxiliary fluorescence or handcrafted steps.

\paragraph{Label-free prediction and nuclear segmentation.}
Early efforts in label-free fluorescence prediction trained convolutional networks to map transmitted-light images directly to fluorescent channels \cite{christiansen2018silico,ounkomol2018label,rivenson2019phasestain}. While effective in 2D, these methods degrade in 3D brightfield volumes, where axial blur and signal ambiguity increase with depth. Instance-segmentation frameworks such as Cellpose \cite{stringer2021cellpose} and its variants include brightfield models, yet they depend on strong morphological priors, 2D processing, or post-hoc volumetric reconstruction to approximate 3D structure. In contrast, our setting is stricter: we predict \emph{3D subcellular structure masks directly from brightfield data}, end-to-end, without auxiliary fluorescence, priors, or handcrafted post-processing.


%\paragraph{U-Net families in 3D.}
%3D U-Net \cite{cciccek20163d}, V-Net \cite{milletari2016v}, UNet++ \cite{zhou2018unet++}, nnU-Net/dynUNet \cite{Isensee_2020} and medical variants of UNETR \cite{hatamizadeh2022unetr} remain strong baselines. Their strengths are locality and scale-space priors, but their receptive field grows diffusely and can be mismatched to confocal anisotropy: axial downsampling and 3D strided convolutions often smear thin structures and introduce block artifacts along $z$. Moreover, capturing long-range correspondences across large $H\!\times\!W\!\times\!D$ contexts typically demands deeper encoders or heavy multi-scale fusion. We address these issues with (i) an \textbf{anisotropic patch embed} that anti-aliases along $z$ before decimation and tiles $xy$ into $2\times 16\times 16$ tokens to match the microscope PSF, and (ii) \textbf{Native Sparse Attention} that injects global context without resorting to fragile, very deep pyramids.

%%BSM minor edits here
%%===============================
\paragraph{U-Net families in 3D.}
3D U-Net \cite{cciccek20163d}, V-Net \cite{milletari2016v}, UNet++ \cite{zhou2018unet++}, nnU-Net/dynUNet \cite{Isensee_2020}, and medical variants of UNETR \cite{hatamizadeh2022unetr} remain strong baselines for volumetric segmentation. Their strengths lie in local feature modeling and scale-space priors, yet their receptive fields expand diffusely and often misalign with confocal anisotropy: axial downsampling and 3D strided convolutions tend to smear thin structures and introduce block artifacts along $z$. Moreover, capturing long-range correspondences across large $H\!\times\!W\!\times\!D$ contexts typically requires very deep encoders or heavy multi-scale fusion. We address these challenges with (i) an \textbf{anisotropic patch embedding} that anti-aliases along $z$ before decimation and tiles $xy$ into $2\times16\times16$ tokens to match the microscope point-spread function (PSF), and (ii) \textbf{Native Sparse Attention} that provides efficient global context without resorting to deep pyramidal hierarchies.


\paragraph{Vision Transformers for medical imaging.}
Transformer backbones such as ViT and DeiT, adapted to segmentation through TransUNet \cite{chen2021transunet}, UNETR \cite{hatamizadeh2022unetr}, and hybrid variants, improve long-range reasoning but suffer from quadratic computational cost. Swin Transformer \cite{liu2021swin} and Swin-UNETR \cite{hatamizadeh2021swin} mitigate this with shifted windows; however, their locality introduces \emph{context barriers}: fine details remain crisp within a window, yet cross-window grouping and long-range axial coherence propagate slowly and require delicate stage tuning. Window parameters are typically optimized for near-isotropic images; under confocal anisotropy, they tend to over-aggregate axially or under-connect laterally. Our \textbf{Native Sparse Attention (NSA)} replaces windowing with a three-branch routing scheme—local sliding, coarse compressed memory, and selected global blocks—allowing tokens to integrate distant context in a single hop while still preserving brightfield-specific edge fidelity.

%\paragraph{Vision Transformers for medical imaging.}
%Transformer backbones (ViT, DeiT) adapted to segmentation via TransUNet \cite{chen2021transunet}, UNETR \cite{hatamizadeh2022unetr} and hybrids improve long-range reasoning but incur quadratic cost. Swin Transformer \cite{liu2021swin} and Swin-UNETR \cite{hatamizadeh2021swin} reduce complexity with shifted windows; however, window locality can create \emph{context barriers}: fine details are crisp within a window, but cross-window grouping and long-range axial agreements propagate slowly and require careful stage design. Window sizes are usually tuned for near-isotropic images; under confocal anisotropy they either over-aggregate axially or under-connect laterally. Our NSA replaces windowing with a three-branch pattern—local sliding, coarse compressed memory, and selected global blocks—so tokens can aggregate distant context in one hop while still modeling local brightfield edges.

%\paragraph{Efficient/sparse attention.}
%Longformer, BigBird, and deformable attention \cite{beltagy2020longformer,zaheer2020big,zhu2020deformable} temper the quadratic cost by structural sparsity or learned sampling. NSA \cite{yuan2025native} (which we adapt to 3D token lattices) combines a fixed local window with \emph{compressive memory} and \emph{top-$k$ selected global blocks}, and learns to mix the three streams per head. To our knowledge, NSA has seen limited use in 3D vision; we show that, with anisotropic tokenization and grouped-query heads, NSA aligns well with the statistics of brightfield volumes: local intensity gradients are handled by the sliding window, coarse axial context is routed through compression, and rare but decisive global cues (e.g., nucleolus contrast, shape priors across slices) are captured by the selected blocks. \bsm{you can make this stronger, by saying somethiong clear and explicit in ".. extend it to 3D anisotropic lattices?"}

\paragraph{Efficient and sparse attention.}
% \bsm{novelty claim re: extension to 3D lattices neetd to be made clear. reworded.}
Longformer, BigBird, and deformable attention \cite{beltagy2020longformer,zaheer2020big,zhu2020deformable} mitigate quadratic cost through structured sparsity or learned sampling. \textbf{Native Sparse Attention (NSA)} \cite{yuan2025native}, which we extend from 2D sequences to \emph{3D anisotropic token lattices}, combines a fixed local window with \emph{compressive memory} and \emph{top-$k$ selected global blocks}, while learning to mix the three streams per head. This reformulation allows NSA to operate natively in volumetric space, aligning its sparsity patterns with the geometry of confocal microscopy data. Local intensity gradients are captured by the sliding window, coarse axial context is routed through compression, and rare but decisive global cues—such as nucleolar contrast or cross-slice morphology—are recovered by the selected blocks. To our knowledge, Bright-4B is the first to demonstrate NSA adapted to 3D anisotropic volumes, providing both scalability and brightfield-specific structural fidelity.


%\paragraph{Stabilizing deep Transformers.}
%Pre-norm and RMSNorm \cite{zhang2019root} reduce training instabilities, but very deep stacks can still drift in scale or gate the wrong paths. Hyper-connections \cite{Zhu2024HyperConnections} add \emph{width} and \emph{depth} gates and per-layer lerp scales, which we adopt to stably blend pre/post updates across multiple residual streams. In parallel, normalized-Transformer ideas (``nGPT'') \cite{loshchilov2024ngpt} motivate training on the unit hypersphere to eliminate scale-chasing; we follow this by $L_2$-normalizing hidden states and projections. The combination gives us depth without gradient brittleness and preserves contrast information critical to brightfield boundaries.

\paragraph{Stabilizing deep Transformers.}
Pre-norm and RMSNorm \cite{zhang2019root} mitigate training instabilities, yet very deep stacks can still drift in scale or misgate residual paths. \textbf{HyperConnections} \cite{Zhu2024HyperConnections} introduce learned \emph{width} and \emph{depth} gates with per-layer interpolation factors, which we adopt to stably blend pre- and post-update states across multiple residual streams. In parallel, normalized-Transformer formulations \cite{loshchilov2024ngpt} motivate learning on the unit hypersphere to suppress scale amplification. We combine these two ideas: all hidden states and projections are $L_2$-normalized so that updates act as rotations on the hypersphere, while HyperConnections control the magnitude and mixing of residual paths. This synergy provides depth without gradient brittleness and preserves the fine contrast essential for accurate brightfield boundary reconstruction.

%\paragraph{Mixture-of-Experts at scale.}
%Sparse MoE models such as GShard and Switch \cite{lepikhin2020gshard,fedus2022switch} scale capacity with conditional computation, but hard routing can be brittle under class imbalance and medical heterogeneity. Soft Mixture-of-Experts (SoftMoE) \cite{puigcerver2023sparse} uses smooth dispatch and learned combination, improving load balance and gradient flow. We employ a \emph{slot-based SoftMoE} in the MLP position: tokens form dynamic slots, experts specialize (e.g., high-frequency edges vs.\ low-frequency textures), and outputs are softly combined and re-normalized. In brightfield, where contrast varies with depth, this conditional capacity lets the network allocate compute to faint structures without overfitting to bright artifacts.

\paragraph{Mixture-of-Experts at scale.}
Sparse MoE architectures such as GShard and Switch \cite{lepikhin2020gshard,fedus2022switch} expand model capacity through conditional computation, but hard routing often proves brittle under class imbalance and medical data heterogeneity. Soft Mixture-of-Experts (SoftMoE) \cite{puigcerver2023sparse} alleviates this with smooth dispatch and learned combination, improving load balance and gradient flow. We extend this formulation with a \textbf{slot-based SoftMoE} operating on the \emph{unit hypersphere}: tokens are grouped into dynamic slots, experts specialize (e.g., high-frequency edges vs.\ low-frequency textures), and outputs are softly recombined and re-normalized. This hyperspherical formulation stabilizes expert routing and prevents scale drift at billion-parameter scale. In brightfield data, where contrast varies sharply with depth, such conditional capacity enables selective computation on faint subcellular structures without overfitting to bright artifacts.


==> sec/3_methods_OG.tex <==
\section{Methods}
%\bsm{gives impression that the contribution is primarily in combination and adaptation, ok but needs to be strengthed to demonstrate that it is more than just putting them together. 

%Also,  show why these components synergize—e.g., ablation tables demonstrating improvements in boundary accuracy, gradient stability, or memory efficiency.}

\paragraph{Overview and design synergy.}
Bright-4B unifies four complementary innovations into a coherent 3D segmentation architecture designed for label-free brightfield data. The \textbf{anisotropic patch embedding} aligns tokenization with the microscope point-spread function, ensuring that axial information is decimated only after PSF-aware anti-alias filtering. These geometry-faithful tokens feed into \textbf{Native Sparse Attention (NSA)}, which routes information through local, coarse, and global paths matched to the spatial statistics of brightfield microscopy. The resulting multi-scale features are processed by a \textbf{slot-based SoftMoE} that operates entirely on the \textit{unit hypersphere}, enabling stable expert specialization without scale drift. Finally, \textbf{Dynamic HyperConnections} blend multiple residual streams through learned width–depth gates, maintaining representation stability across billion-parameter depth. Together, these modules form a hyperspherical learning stack in which attention, expert routing, and residual mixing occur within a single normalized manifold—yielding sharper subcellular boundaries, improved gradient stability, and efficient 3D reasoning beyond what any component achieves in isolation.

\subsection{Problem Setup and Notation}

%The problem we are trying to solve is voxelwise subcellular structure segmentation from 3D brightfield microscopy. Given a volume $x \in \mathbb{R}^{B\times C\times D\times H\times W}$ (batch $(B)$, channels $(C)$, axial depth $(D)$, in-plane size $(H\times W)$, the goal is to predict a binary mask $y \in \{0,1\}^{B\times 1\times D\times H\times W}$. We partitioned the volume with an anisotropic patch size $P=(p_z,p_y,p_x)=(2,16,16)$. After anti-aliasing and striding in $z$, and tiling in $xy$, the token lattice has spatial shape $D'=\frac{D}{p_z}$, $H'=\frac{H}{p_y}$, $W'=\frac{W}{p_x}$ and $N=D'H'W'$ tokens. Each token is projected to a hidden size $(h=512)$, yielding $T \in \mathbb{R}^{B\times N\times h}$.  Divisibility constraints $(D\mod p_z=H\mod p_y=W\mod p_x=0)$ are enforced by patch cropping.
We address the task of voxelwise subcellular structure segmentation from 3D brightfield microscopy volumes. Given an input volume $x \in \mathbb{R}^{B\times C\times D\times H\times W}$—with batch size $B$, channels $C$, axial depth $D$, and in-plane dimensions $(H\times W)$—the goal is to predict a binary segmentation mask $y \in \{0,1\}^{B\times 1\times D\times H\times W}$. The volume is partitioned into anisotropic patches of size $P=(p_z,p_y,p_x)=(2,16,16)$. After PSF-aware anti-aliasing and striding along $z$, and tiling in the $xy$ plane, the resulting token lattice has spatial dimensions
$D'=\tfrac{D}{p_z}$, $H'=\tfrac{H}{p_y}$, $W'=\tfrac{W}{p_x}$, and $N=D'H'W'$ tokens. Each patch is linearly projected to a hidden dimension $h=512$, yielding a token tensor $T \in \mathbb{R}^{B\times N\times h}$. Divisibility constraints $(D\bmod p_z = H\bmod p_y = W\bmod p_x = 0)$ are enforced through boundary cropping.

The backbone is a 12-layer normalized Transformer with eight attention heads and a soft Mixture-of-Experts (MoE) module (72 experts, expansion factor 8) replacing the standard MLP; dropout is set to 0.1. All hidden states are $L_2$-normalized, so each block performs rotations on the unit hypersphere rather than unconstrained rescalings. The decoder follows a UNETR-style \cite{hatamizadeh2022unetr} pyramid with a base feature size of 64, reshaping intermediate token maps back to $(D'\!\times\!H'\!\times\!W')$ and progressively upsampling to full spatial resolution.

Patch and embedding parameters were empirically optimized for brightfield microscopy data. Brightfield structure is information-rich at micron-scale in-plane but comparatively sparse along the axial dimension. Setting $(p_z{=}2)$ preserves thin axial features, while $(p_y{=}p_x{=}16)$ aggregates local texture into manageable tokens, balancing aliasing suppression and computational load. 

% For a typical field of view $(32\times128\times128)$, this configuration yields $(N=(32/2)\cdot(128/16)\cdot(128/16)=1024)$ tokens. With a hidden size of $h{=}512$, the resulting token tensor $(B\times1024\times512)$ fits comfortably within a single GPU and keeps self-attention complexity sub-quadratic under the applied sparsity.

%The backbone is a 12-layer normalized Transformer with 8 attention heads and a soft Mixture-of-Experts (MoE) (72 experts, expansion 8) in place of the MLP; dropout is 0.1.  All hidden states are L2-normalized, so blocks act as rotations on the unit hypersphere rather than rescalings.  The decoder is a UNETR-style \cite{hatamizadeh2022unetr} pyramid with base feature size 64 that reshapes intermediate token maps back to $(D'\times H' \times W')$ and progressively upsamples to full resolution. 

%These shapes were tested and chosen specifically for microscopy data. Brightfield structure is rich at micron-scale in-plane but sparse axially; $(p_z{=}2)$ preserves thin axial features while $(p_y{=}p_x{=}16)$ amortizes local texture into tokens, balancing aliasing and compute. For a typical patch of $(32\times 128\times 128)$, this yields $(N=(32/2)\cdot(128/16)\cdot(128/16)=1024)$ tokens; with $(h{=}512)$, the token tensor is $(B\times 1024\times 512)$, which fits comfortably on a single GPU and keeps attention sub-quadratic under sparsity. 

% *Outputs and losses.* The network outputs a logit volume (\hat{y}\in\mathbb{R}^{B\times 1\times D\times H\times W}); we use a sigmoid at inference and segmentation losses (§Training) during learning. *[Mechanism → Evidence]*

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{sec/figs/HYPER.pdf}
    \caption{ \textit{Hypersphere Setup.} \textbf{[A]} The pre-update $x_0$ and proposal $\hat{u}$ live on the unit sphere. We use LERP and L2 Normalization (chord + radial projection) which is approximately SLERP for small angles. \textbf{[B]} Given the sublayer output from MoE or Attention, we take small, feature-wise steps which are stable on the hypersphere. \textbf{[C]} We use a two-input mixer with gat $\beta$ blending in $\mathbb{R}^d$ Depth gate arbiters new evidence versus prior memory per feature. \textbf{[D]} Process $E$ streams in parallel, then reduce outputs and normalize. Simply put: Width = multiple latent opinions, merge = consensus on the hypersphere.}
    \label{fig:hypersphere}
\end{figure}


\subsection{Anisotropic Patch Embedding}

We tokenize 3D brightfield volumes using an anisotropy-aware patch embedding module that aligns with the microscope point-spread function (PSF). Given an input volume $x \in \mathbb{R}^{B\times C\times D\times H\times W}$, we first apply a depthwise 3D convolution with kernel $(p_z,1,1)$, stride $(p_z,1,1)$, and groups $=C$ to low-pass filter and subsample only along the axial direction. This PSF-aware anti-aliasing preserves thin axial structures before decimation, producing $x' \in \mathbb{R}^{B\times C\times D'\times H\times W}$, where $D' = D/p_z$. 

Next, we fold non-overlapping $xy$ tiles of size $(p_y,p_x)$ into token channels: $
\text{rearrange}(x') : (B,C,D',H,W) \rightarrow (B,D',H',W',p_y p_x C),
$
where $H' = H/p_y$ and $W' = W/p_x$. Each token vector $\in \mathbb{R}^{p_y p_x C}$ is mapped to a latent dimension $h$ by a bias-free linear projection, yielding a 3D token lattice $\in \mathbb{R}^{B\times D'\times H'\times W'\times h}$. 

Importantly, $p_z$ does not appear in the token dimension, since axial downsampling is handled entirely by the anti-alias convolution. This preserves precise spatial indexing and makes the module a drop-in replacement for standard \texttt{rearrange}+linear patchifiers. This simple three-step sequence—anti-alias and stride in $z$, tile in $xy$, and project to $h$—minimizes aliasing, respects confocal anisotropy, and produces geometry-faithful tokens for downstream 3D attention and UNETR decoding.


%We tokenize 3D confocal volumes with an anisotropy-aware patch embed that matches the microscope’s point-spread function (PSF). Given $x\in\mathbb{R}^{B\times C\times D\times H\times W}$, we first low-pass and subsample only along the axial direction using a depthwise 3D convolution with kernel $(p_z,1,1)$, stride $(p_z,1,1)$, and groups $=C$. This PSF-aware anti-aliasing preserves thin axial structures before decimation, yielding $x'\in\mathbb{R}^{B\times C\times D'\times H\times W}$ with $D'=D/p_z$. We then fold non-overlapping XY tiles of size $(p_y,p_x)$ into token channels: $\text{rearrange}(x'):(B,C,D',H,W)\!\rightarrow\!(B,D',H',W',p_y p_x C)$, where $H'=H/p_y,\,W'=W/p_x$. Each token vector $\in\mathbb{R}^{p_y p_x C}$ is mapped to a latent dimension $h$ by a bias-free linear projection (NormLinear), producing a 3D token lattice $\in\mathbb{R}^{B\times D'\times H'\times W'\times h}$. Note that $p_z$ does not appear in the token dimension (downsampling in $z$ is handled by the axial conv), which keeps spatial indexing exact and makes the module a drop-in replacement for rearrange+linear patchifiers. This simple sequence—anti-alias then stride in $z$, tile in $xy$, project to $h$—reduces aliasing, respects confocal anisotropy, and yields geometry-faithful tokens for downstream 3D attention and UNETR decoding.

% \begin{figure}
%     \centering
%     \includegraphics[width=1\linewidth]{sec/figs/anisotropic.pdf}
%     \caption{\textbf{DRAFT FIGURE} \textit{Anisotropic 3D patch embedding.} We first apply a PSF-aware depthwise axial low-pass with stride $p_z$ to prevent aliasing, yielding $(B, C, D/p_z, H, W)$. We then tile the $XY$ plane into $p_y \times p_x = 16\times16$ blocks and fold each tile (across channels) into a vector of length ($p_y p_x C$). A bias-free projection maps each vector to (h) dimensions, producing a geometry-faithful token lattice ($(B, D', H', W', h)$) with ($D' = D/2$). Crucially, $p_z$ does not inflate the token dimension; axial decimation is handled by the anti-alias conv, while token content remains $(16\times16\times C)$. This $(2\times16\times16)$ design respects confocal anisotropy and reduces block artifacts, yielding crisp boundaries in downstream 3D segmentation.
% }
%     \label{fig:placeholder}
% \end{figure}

% \subsection{Sparse Attention}

% Each transformer block replaces dense self-attention with a three-branch sparse module \cite{yuan2025native} that mixes (i) a local sliding window over nearby tokens, (ii) a coarse global pathway that attends to compressed key–values, and (iii) a fine global pathway that selectively attends to a few high-salience remote blocks. Concretely, let $X\in\mathbb{R}^{B\times N\times d}$ be unit-norm tokens, split into $(H)$ heads with head size $(d_h)$. For each head we compute
% \begin{align}
%     Y_{\text{local}}&=\text{Attn}\big(Q,K_{t\pm w/2},V_{t\pm w/2}\big),\\
% Y_{\text{coarse}}&=\text{Attn}\big(Q,\tilde K,\tilde V\big),\\
% Y_{\text{fine}}&=\text{Attn}\big(Q,K_{\mathcal S},V_{\mathcal S}\big),
% \end{align}
% where $w$ is the 1D window size, $\tilde K,\tilde V$ are compressed features obtained by splitting the sequence into overlapping blocks and mapping each block through a small Compression Transformer ((4) layers, width $d_h \times \texttt{kv\_heads}=1024)$, and $\mathcal S$ is the set of top-$k$ remote blocks selected by the coarse attention scores. The three branches are merged per head by a learned sigmoid mixer $\alpha\in[0,1]^3$ (initialized to prefer local), giving
% \begin{align}
% Y = \sum_{s\in{\text{coarse},\text{fine},\text{local}}} \alpha_s , Y_s,\quad Y\in\mathbb{R}^{B\times N\times d_h}.
% \end{align}
% We use grouped-query attention (GQA) \cite{ainslie-etal-2023-gqa} with $\texttt{kv\_heads}\le H$ to reduce KV memory.

% % Instantiation for our token lattice, might add one more sentence

% With $(D,H,W)=(32,128,128)$ and patches $(p_z,p_y,p_x)=(2,16,16)$, the anisotropic embed yields a $(16\times 8\times 8)$ grid, \ie  $N=1024$ tokens. We set head size $d_h=128$, $H=8$, thus $d=512$. We chose a sliding window size of 256 because this covers a compact 3D neighborhood under the row-major flattening used by the embed, so most tokens within a nucleus and its immediate membrane contrast fall inside the same window. For the compression block size, we went with 32 and a stride of 16, which is a 50 percent overlap, giving us 64 course blocks over the sequence. Each block is summarized by the compression transformer into $\tilde K,\tilde V$ plus 8 learned memory slots, giving a low-rank global map of illumination, background texture, and slice-wise trends. Brightfield images are dominated by local phase-contrast cues at nuclear boundaries (thin, high-frequency), slow, global fields (illumination ramps, stage/vignetting) that can confound local gradients, and sparse, long-range dependencies(\eg consistent morphology across slices or repeating structures). Dense attention wastes compute on irrelevant long-range pairs. Purely local attention misses cross-slice/global corrections.

% Because states and projections are unit-norm \cite{loshchilov2024ngpt}, attention steps are directional updates on a hypersphere \cite{tongzhouw2020hypersphere}. NSA’s mixer produces bounded convex combinations of three well-conditioned branches; HyperConnections \cite{Zhu2024HyperConnections} then interpolate each layer’s pre/post state with learned lerp scales. Empirically this prevents over-confident global jumps (a known failure mode when global context is noisy in brightfield) and keeps optimization stable at depth.

\begin{figure}
    \centering
    \includegraphics[width=0.6\linewidth]{sec/figs/ARCH.pdf}
    \caption{\textbf{Bright 4B Architecture.} Each block follows PreNorm-Attention-Residual and PreNorm-FFN-Residual, but with two additions: a cross-stream mixer that blends E residual streams, and a spherical residual gate that applies unit-norm LERP updates. We replace MHA with Native Sparse Attention (sliding window, compressed memory, global selection) and the MLP with Soft-MoE (slot-based soft routing + load balancing). Shapes are preserved $(B, N, d)$ throughout.}
    \label{fig:placeholder}
\end{figure}


\subsection{Native Sparse Attention on 3D Token Lattices}

We instantiate the Native Sparse Attention (NSA) \cite{yuan2025native} framework on the vision tokens produced by our anisotropic patch embedding. Let $\mathbf{H}\!\in\!\mathbb{R}^{m\times d}$ be the token matrix ( $m$ tokens, $d$ channels ) and let $(\mathbf{Q},\mathbf{K},\mathbf{V})$ be standard projections. Rather than attending to all $\mathbf{K},\mathbf{V}$, NSA \emph{remaps} them into a compact, information-dense set that depends on the current query and a contextual memory. Formally, for a query at position $t$ we construct representation pairs
$\widetilde{\mathbf{K}}_t\!=\!f_K(\mathbf{q}_t,\mathbf{k}_{1:t},\mathbf{v}_{1:t}),
\widetilde{\mathbf{V}}_t\!=\! f_V(\mathbf{q}_t,\mathbf{k}_{1:t},\mathbf{v}_{1:t}),
$
and compute the attention proposal $  \mathbf{o}_t^{\star} = \text{Attn}\!\big(\mathbf{q}_t,\widetilde{\mathbf{K}}_t,\widetilde{\mathbf{V}}_t\big).$
Following the NSA design, we realize $f_K,f_V$ as a \emph{mixture of three mapping strategies} $\mathcal{C}\!=\!\{\text{cmp},\text{slc},\text{win}\}$: (i) \textbf{compression} (cmp) that aggregates sequential blocks into block-level keys/values, (ii) \textbf{selection} (slc) that expands a small set of high-salience blocks back to token resolution, and (iii) a \textbf{sliding window} (win) that preserves a local neighborhood. A per-query gate $\mathbf{g}_t\!\in\![0,1]^3$ (sigmoid MLP on $\mathbf{q}_t$) mixes the three routes.
% \begin{align}
% \mathbf{o}_t^{\star} \;=\; \sum_{c\in\mathcal{C}} g_t^{c}\;\text{Attn}\!\big(\mathbf{q}_t,\widetilde{\mathbf{K}}^{c}_t,\widetilde{\mathbf{V}}^{c}_t\big), \qquad
% \sum_{c} g_t^{c}=1. \label{eq:nsa-mix}
% \end{align}
The total number of remapped keys is therefore highly sparse, yielding sub-quadratic complexity.
% \begin{align}
% N_t \;=\; \sum_{c\in\mathcal{C}}\big|\widetilde{\mathbf{K}}^c_t\big| \;\ll\; t,
% \end{align}


\paragraph{Token compression.}
The goal of the compression pathway is to provide denoised, long-range context without importing background clutter or inflating computational cost. We replace thousands of past tokens with a compact set of semantic anchors—coarse ``tiles'' corresponding to recurring structures such as nuclear or organelle clusters—computed by a lightweight Transformer. All compressed states are constrained to lie on the same unit hypersphere as the local tokens, ensuring that downstream attention and depth updates remain scale-stable.


%The goal of the compression pathway is to supply denoised, long-range context without importing background clutter or blowing up compute. We replace thousands of past tokens with a small set of semantic anchors (coarse ``tiles" such as nuclear clusters or (\ak{CANT THINK OF ANYTHING HERE)}) computed by a light Transformer, and we ensure all compressed states live on the same unit hypersphere as the local tokens so that downstream attention and depth updates remain scale-stable.

We partition past keys/values into blocks of length $B$ with stride $S$ and map each block to one compressed key/value with a light \emph{Compression Transformer} $\phi$ (3 layers, $256$ dim, $k_v$ heads). The tiny transformer $\phi$ acts as a semantic low-pass: short-context self-attention with Pre-Norm and residuals preferentially preserves patterns consistent across a block (nuclear clusters, organelle fields) and suppresses high-frequency BF speckle.
% (50\% overlap). Overlap mitigates information fragmentation when nuclei span block boundaries; the compressor learns coarse semantic ``tiles" (nuclear clusters, cytoplasm fields, halos) that serve as memory anchors.

\paragraph{Token selection.}
Given compressed logits $\mathbf{s}_t\!\in\!\mathbb{R}^{\lceil t/S\rceil}$ computed as softmaxed dot products between $\mathbf{q}_t$ and $\widetilde{\mathbf{K}}^{\text{cmp}}_t$, we select $\kappa$ top blocks and \emph{expand} them back to tokens with block size $L$ (we use $L\!=\!32$, $\kappa\!=\!8$).
% \begin{align}
% \mathcal{J}_t = \text{TopK}(\mathbf{s}_t,\kappa),\\
% \widetilde{\mathbf{K}}^{\text{slc}}_t = \text{concat}\big\{\mathbf{K}_{J:L}\;|\;J\!\in\!\mathcal{J}_t\big\}, \\
% \widetilde{\mathbf{V}}^{\text{slc}}_t = \text{concat}\big\{\mathbf{V}_{J:L}\;|\;J\!\in\!\mathcal{J}_t\big\}. \label{eq:slc-map}
% \end{align}
This path yields high-fidelity long-range evidence only where needed (\eg, elongated nuclei, mitotic events), avoiding quadratic cost.

\paragraph{Sliding window.}
Finally, we preserve a fixed local neighborhood of radius $W$ around $t$,
% \begin{align}
% \widetilde{\mathbf{K}}^{\text{win}}_t=\mathbf{K}_{t-W:t+W}, \\
% \widetilde{\mathbf{V}}^{\text{win}}_t=\mathbf{V}_{t-W:t+W},
% \end{align}
with $W\!=\!256$ tokens. This route stabilizes gradients, captures boundaries and phase edges, and acts as a strong prior for brightfield where most cues are local.

\paragraph{Grouped queries and normalization.}
We employ grouped-query attention \cite{ainslie-etal-2023-gqa} ($k_v$ heads $\le$ heads) so multiple query heads share the same remapped $\widetilde{\mathbf{K}},\widetilde{\mathbf{V}}$, reducing memory while encouraging consistent global decisions across heads. The NSA output $\mathbf{o}_t^{\star}$ is \emph{normalized} and combined via a diagonal spherical lerp update \cite{shoemake1985animating}, preventing any branch from winning by scale and improving mixed-precision stability.

\paragraph{Why NSA fits brightfield.}
% Brightfield volumes exhibit anisotropy, halos, and depth-dependent blur. NSA’s three routes map neatly onto these phenomena: sliding windows preserve crisp edges and near-field interference; compression aggregates blurry but informative mesoscale context across depth; selection restores only the distant regions that a query deems salient (e.g., long nuclear spines), side-stepping noise elsewhere. Our settings ($B\!=\!32,S\!=\!16,L\!=\!32,\kappa\!=\!8,W\!=\!256$) align with typical nucleus diameters and inter-nuclear spacing in our token lattice, yielding the best compute–accuracy tradeoff we found. Empirically, NSA reduces block artifacts and recovers sharper, depth-consistent boundaries compared to dense attention or window-only variants, while remaining tractable at 3D resolutions.

Brightfield volumes exhibit $z$-anisotropy (PSF blur), halos, and clutter. NSA’s three routes map cleanly to these phenomena: the sliding window preserves crisp edges and near-field interference; the compression pathway aggregates blurry but informative mesoscale context across depth (a semantic low-pass); and the selection pathway restores only \emph{distant} high-fidelity regions judged salient by the query, side-stepping background noise. Our parameters $(B{=}32,\, S{=}32\ \text{main}/16\ \text{ablation},\, L{=}64,\, \kappa{=}4,\, W{=}128)$ match typical subcellular structure extents and spacing on our token lattice, yielding a strong compute–accuracy trade-off. Empirically, NSA reduces block artifacts and recovers sharper, depth-consistent boundaries versus dense attention or window-only variants—while remaining tractable for 3D.







% * The local window captures edge/texture evidence needed to delineate membranes and suppress blockiness; on our 3D grid, (w{=}256) comfortably encloses typical nucleus diameters plus margin.
% * The coarse branch builds a global, low-rank model of nuisances (illumination/background) via learnable compression; attention to (\tilde K,\tilde V) lets each token subtract global bias before edge integration, reducing halo artifacts that plague brightfield segmentation.
% * The **fine branch** focuses compute on a **few** remote regions most predictive for the current token (top-k blocks). In practice, these often correspond to adjacent slices or homologous textures; bringing exactly those into the receptive field sharpens boundaries without quadratic cost.

% With (N{=}1024), the branch budgets above yield ~(,w(=256) + k\cdot s(=256) + \text{mem}(≲64),) candidate keys per query—**≈576** effective context tokens instead of 1024—cutting attention FLOPs by ~(2\times) while **increasing** the *useful* context (local + selected) relative to uniform dense attention. The overlap (c{:}\text{stride}=32{:}16) stabilizes coarse summaries (each fine block is seen in two compress windows), and (k{=}8) balances recall of rare but relevant regions with over-selection noise. Head size (128) aligns with the CompressTransformer width ((d_h\times\text{kv_heads}=1024)), avoiding representational bottlenecks.

% Because states and projections are unit-norm (nGPT-style), attention steps are **directional updates on a hypersphere**. NSA’s mixer produces bounded convex combinations of three well-conditioned branches; HyperConnections then interpolate each layer’s pre/post state with learned lerp scales. Empirically this prevents over-confident global jumps (a known failure mode when global context is noisy in brightfield) and keeps optimization stable at depth.


% -----------------------------
% CHATGPT answer, need to check

% Per token, the cost is (O\big(H,[,w + k,s + m,]\big)) for window (w), selected fine tokens (k,s), and a small memory (m) from compression—versus (O(HN)) for dense attention. Here that is (O(8\times!576)) instead of (O(8\times!1024)), with much better context quality.

% -----------------------------


% To our knowledge, prior 3D medical vision works rely on local/windowed, axial, or block-sparse attention; our module is the first to **port DeepSeek’s Native Sparse Attention to 3D volumes**, and to **couple** it with (i) *learned* compressive summaries (a miniature transformer rather than pooling), (ii) *hypersphere* normalization (nGPT) and (iii) *HyperConnections* for depth-wise stability, all **inside a ViT–UNETR** tailored to confocal anisotropy. This combination lets the model separate local boundary evidence from global nuisance fields and selectively import long-range support, which we find crucial for crisp nuclei in brightfield.

% We use (H{=}8), (d_h{=}128), (w{=}256); compression (c{=}32), stride (16), memory (8); fine selection (s{=}32), (k{=}8); (\text{kv_heads}{=}8) with shared selection across grouped queries; the CompressTransformer has 4 layers and width (1024). The attention mixer is initialized to favor the local branch, letting the model ``earn" global context as training progresses.







\subsection{Soft Mixture of Experts}

We replace the feed-forward block with a \emph{Soft MoE} layer \cite{puigcerver2023sparse} that grows capacity without increasing per-token compute. Let the token matrix be $\mathbf{X}\in\mathbb{R}^{m\times d}$ ( $m$ tokens, $d$ channels ). The layer owns $n$ experts, each applied to $p$ \emph{slots}, for a total of $s=n\!\cdot\!p$ slots. A learned key matrix $\boldsymbol{\Phi}\in\mathbb{R}^{d\times s}$ produces routing logits; a column-wise softmax yields \emph{dispatch} weights $\mathbf{D}\in\mathbb{R}^{m\times s}$ that convex-combine tokens into slots.
% \begin{align}
% \mathbf{D}_{ij} &= \frac{\exp\!\big((\mathbf{X}\boldsymbol{\Phi})_{ij}\big)}{\sum_{i'=1}^{m}\exp\!\big((\mathbf{X}\boldsymbol{\Phi})_{i'j}\big)}, \quad
% \tilde{\mathbf{X}} = \mathbf{D}^\top \mathbf{X}\in\mathbb{R}^{s\times d}. \label{eq:dispatch}
% \end{align}
Each expert $f_k:\mathbb{R}^{d}\!\rightarrow\!\mathbb{R}^{d}$ processes its $p$ assigned rows of $\tilde{\mathbf{X}}$, producing slot outputs $\tilde{\mathbf{Y}}\in\mathbb{R}^{s\times d}$. Tokens are then reconstructed by a \emph{combine} step that uses a row-wise softmax over the same logits to form weights $\mathbf{C}\in\mathbb{R}^{m\times s}$.
% \begin{align}
% \mathbf{C}_{ij} &= \frac{\exp\!\big((\mathbf{X}\boldsymbol{\Phi})_{ij}\big)}{\sum_{j'=1}^{s}\exp\!\big((\mathbf{X}\boldsymbol{\Phi})_{ij'}\big)}, \quad
% \mathbf{Y} = \mathbf{C}\,\tilde{\mathbf{Y}}\in\mathbb{R}^{m\times d}. \label{eq:combine}
% \end{align}
Both \textit{dispatch} and \textit{combine} are convex: slots are weighted averages of tokens, and tokens are weighted averages of expert outputs. 
% In practice we set $s$ to match the FLOPs of a dense MLP layer; a light load-balancing term encourages high-entropy routing and prevents expert collapse,
% \begin{align}
% \mathcal{L}_{\text{lb}} = \lambda \big( \underbrace{\text{H}_{\text{row}}(\mathbf{C})}_{\text{balanced combine}} +  \underbrace{\text{H}_{\text{col}}(\mathbf{D})}_{\text{balanced dispatch}} \big),
% \end{align}
% where $\text{H}$ denotes mean entropy over rows/columns. 
All vectors are unit-normalized, so experts operate on the hypersphere and cannot solve the task by inflating feature scales.

\paragraph{Why MoE helps brightfield.}
Brightfield volumes exhibit high heterogeneity: weak edges, phase halos, uneven illumination, and morphology that couples distant voxels. Soft MoE addresses these challenges in three ways. \textit{(i) Noise-robust aggregation.} The slotting $\tilde{\mathbf{X}}=\mathbf{D}^\top\mathbf{X}$ performs adaptive, content-aware averaging before expertise is applied; this suppresses speckle and halo noise while preserving coherent structure, improving boundary sharpness after the decoder. \textit{(ii) Specialization without dead experts.} Because routing is soft (every token contributes to many slots with small weights) and gradients flow through $\mathbf{D}$ and $\mathbf{C}$, experts naturally specialize (e.g., thin rims, dense chromatin, defocused planes) without the brittleness of hard top-$k$ gating. \textit{(iii) Capacity at fixed compute.} With $s$ chosen to match a dense MLP, the layer increases representational diversity (via $n$ experts) yet keeps per-token FLOPs unchanged; this is crucial for long 3D sequences where attention already consumes memory. In our stack, native sparse attention supplies local/coarse/global context, and Soft MoE converts these features into task-specific subroutines—denoising, edge sharpening, and morphology reasoning—on the unit hypersphere, yielding accurate subcellular boundaries from brightfield alone.

\subsection{Dynamic Hyper-Connections}
\label{sec:hc}

In a 4B-parameter backbone that blends native sparse attention (NSA) and SoftMoE, simple residual wiring \cite{he2016deep} is brittle: one route (e.g., the local window) can dominate early, experts can collapse, and scale drift creates unstable optimization—especially in half precision. \emph{Dynamic Hyper-Connections} (DHC) \cite{Zhu2024HyperConnections} address this by (i) running $E$ parallel residual streams that let distinct computations specialize (local, coarse, global/expert), and (ii) learning input-conditioned \emph{width} and \emph{depth} gates that arbitrate among streams while preserving unit-norm geometry. Intuitively, DHC separates ``what to combine" (width mixing across streams) from ``how far to move" (depth interpolation on the hypersphere), preventing any single branch from winning by scale.


\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{sec/figs/results_resid.pdf}
    \caption{For each model, we visualize the predicted mask (Left), and the voxel-wise difference between the pseudolabel and the predicted mask (Right).}
    \label{fig:placeholder}
\end{figure}


\begin{figure*}[!t]
    \centering
    \includegraphics[width=0.95\linewidth]{sec/figs/RESULTS.pdf}
    \caption{\textbf{Qualitative Segmentation Results for Bright 4B}. The first column shows a representative 2D slice from the 3D bright-field input. The remaining columns display our model's segmentation predictions at three distinct z-slices. The z-slice index is indicated in the yellow box, with lower indices corresponding to the bottom of the cell and higher indices to the top. Image width is approximately $97\mu m$.}
    \label{fig:placeholder}
\end{figure*}

\section{Experimental Results}

\paragraph{Dataset} We evaluate our method on the publicly available dataset that comprises over 18,000 3D images of live, human induced pluripotent stem cells (hiPSCs, line WTC-11) spanning 25 fluorescently tagged cellular structures ~\cite{viana2023integrated}. Cells were imaged in tightly-packed epithelial-like colonies using spinning-disk confocal microscopy, with each image containing channels for the tagged structure, cell membrane, and DNA. Further, to enable quantitative image and data analyses, accurate and robust segmentations for all 25 intracellular 3D structure localization patterns were created using the Allen Cell \& Structure Segmenter \cite{Chen491035}. In this work, we have used 5 structures for evaluation: 1)~nucleioli-GC tagged via NPM1, 2)~mitochondria tagged via TOMM20, 3)~microtubules tagged via TUBA1B, 4)~DNA labeled with DNA dye, and 5)~Golgi tagged via ST6GAL1. The 3D images used here have size $924\times624\times65$ or $900\times600\times70$ in the $x$, $y$, and $z$ with pixel size of $0.1083\mu m$ and z-spacing of  $0.29\mu m$.

\iffalse
\sm{overall results. Explanation of main results table. We need to explain the limitations of pseudo-labels here. 

In observations we need to explain why for some structures results look better compared to others- some insight.}

\sm{ablation analysis and more observations regarding contributions}
\fi

\subsection{Nucleoli}

\sm{We first tested our methodology on nucleoli, an organelle chosen because its fluorescent signal is known to be highly predictable from bright-field \cite{ounkomol2018label}. Our results confirm that the model can successfully predict both the location and the overall morphology of individual nucleoli. A key finding is that this predictive accuracy is robust and consistent across the entire z-stack. We did identify a limitation in resolving fine, complex features: the model, for example, tends to miss small internal "holes" (or vacuoles) that are visible in the ground-truth segmentations.}

\subsection{Mitochondria}

\sm{We next evaluated our model on mitochondria, which we selected as an ideal intermediate validation target. This organelle poses a distinct challenge: its refractive index is significantly lower than that of nucleoli, resulting in a low-contrast signal, yet its tubular structures remain resolvable (i.e., above the diffraction limit).

Our model demonstrates high fidelity in this low-signal regime. It not only predicts the 3D location of the mitochondrial network—with high consistency at peripheral z-slices (top and bottom of the cell)—but also accurately resolves the orientation of individual tubules in sparse regions. This ability to capture fine-grained orientation from a convolved, low-contrast input strongly suggests the model is implicitly learning to invert the optical path and perform an effective deconvolution of the bright-field point spread function (PSF).}

\subsection{Microtubules}

\sm{Microtubules, as 25nm sub-diffraction-limit structures, are physically invisible in bright-field microscopy, thus representing the ultimate zero-signal challenge for our model. As hypothesized, the model is unable to reconstruct the fine-grained microtubule network. However, the analysis of this failure case provides a critical insight: rather than producing random noise, the model learns a powerful structural prior.

We observe that its (failed) predictions are correctly confined to the cytoplasmic space and are strictly excluded from the nucleus. This demonstrates that in the total absence of a target signal, the model defaults to learning the valid spatial context of the task. One might hypothesize that microtubule bundles, which are larger and sometimes visible in bright-field (e.g., the mitotic spindle), would be reconstructed. However, our model also fails to resolve these structures in mitotic cells. We attribute this failure to extreme class imbalance: mitotic cells represent only ~$5\%$ of our training data, making them heavily undersampled. The model is thus not exposed to sufficient examples to learn this distinct morphological state.}

\subsection{Conclusion}

\sm{We have presented Bright 4B, a 4-billion parameter foundation model for 3D bright-field segmentation that operates on the unit hypersphere. Our core technical contribution is an anisotropy-aware patch embedding module that aligns with the microscope's PSF. We demonstrated that this approach yields segmentations with high z-axis consistency and accurate organelle localization, particularly for structures with strong optical signals (e.g., high refractive index or supra-diffraction-limit size).

The clear next step is to move beyond pixel-level validation to quantitative biological analysis. Future work must rigorously assess the model's fidelity in downstream tasks, such as measuring nucleolar volume or mitochondrial tubule length.

Furthermore, we found that even in zero-signal regimes like microtubules, the model learns a powerful spatial prior, correctly segmenting the valid cytoplasmic space. Exploring the utility of this implicit nuclear and cellular boundary detection is, in itself, a promising new research direction.}

We benchmark our model using a subset of the data, specifically the mitochondria, since it is not directly visible in bright field, but the filaments are not as thin, making the light scattering pattern enough to learn, and a reasonable level of difficulty as a benchmark. We used 2K FOVs to train each of the architectures. 

\begin{table}
\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}lllll@{}}
\toprule
Architecture          & \# Param & IMF &  &  \\ \midrule
UNET                  & 438M     & 20GB      &  &  \\
Dynamic UNET          & 91M      & 51GB      &  &  \\
UNETR                 & 211M     & 81GB          &  &  \\ 
SWIN UNETR (ISO)      & 248M     & 110GB          &  &  \\
SWIN UNETR (ANISO)    & 247M     & 97GB         &  &  \\
Bright 4B (Our Model) & 4B       & \ws{26GB}      &  & 
\\ \midrule
\end{tabular}%
}
\caption{For each model, we show the empirically chosen parameter counts and inference memory footprint (IMF) that gave the best results for each architecture.}
\label{tab:arch}
\end{table}


% \begin{figure}
%     \centering
%     \includegraphics[width=1\linewidth]{sec/figs/results_resid.pdf}
%     \caption{For each model, we visualize the predicted mask (Left), and the pseudolabel minus predicted mask (Right).}
%     \label{fig:placeholder}
% \end{figure}


\paragraph{Architectural Evaluation}

We chose the number of parameters for each model based on empirical testing to make the comparison between our four billion parameter model as fair as possible. These parameter counts were the most effective for learning the mitochondria structure, and we found that anything below or above these either degraded the performance or added more compute with little to no gain in segmentation accuracy. More precisely, we noticed that for the base UNET, adding more parameters produced more blobby structures and focus shifted more on overall shape, while too few parameters learned the inherent brightfield noise. For the transformer-based models, produced reasonable results all within the $\approx 200M$ range. \ref{tab:arch}

% \bsm{lacks quantitative results, figures, metrics (IoU, Dice, mAP, etc.), or comparisons. highly incomplete for CVPR. Evaluation on public benchmarks? (Allen Cell or ISBI datasets?). Ablation studies as approrpirate. Empirical evidenbce needed to support any strong claims./}

\iffalse
\section{Conclusions}
We present Bright 4B, a 4B-parameter foundation model for segmenting subcellular structures in 3D brightfield microscopy images that learns on the unit hypersphere. Bright 4B produces morphology-accurate segmentations of nucleoli, mitochondria, and other organelles from 3D brightfield stacks. The effectiveness of our approach makes it well-suited for brightfield-based downstream organelle analysis.
\fi
